Complete homotopy invariants for translation invariant symmetric quantum walks on a chain

We provide a classification of translation invariant one-dimensional quantum walks with respect to continuous deformations preserving unitarity, locality, translation invariance, a gap condition, and some symmetry of the tenfold way. The classification largely matches the one recently obtained (arXiv:1611.04439) for a similar setting leaving out translation invariance. However, the translation invariant case has some finer distinctions, because some walks may be connected only by breaking translation invariance along the way, retaining only invariance by an even number of sites. Similarly, if walks are considered equivalent when they differ only by adding a trivial walk, i.e., one that allows no jumps between cells, then the classification collapses also to the general one. The indices of the general classification can be computed in practice only for walks closely related to some translation invariant ones. We prove a completed collection of simple formulas in terms of winding numbers of band structures covering all symmetry types. Furthermore, we determine the strength of the locality conditions, and show that the continuity of the band structure, which is a minimal requirement for topological classifications in terms of winding numbers to make sense, implies the compactness of the commutator of the walk with a half-space projection, a condition which was also the basis of the general theory. In order to apply the theory to the joining of large but finite bulk pieces, one needs to determine the asymptotic behaviour of a stationary Schr\"odinger equation. We show exponential behaviour, and give a practical method for computing the decay constants.

==> 015-results.tex <==
\subsection{Overview of results}

After fixing the setting and the notation used in this publication we establish an equivalence between essential locality of walks under consideration and continuity of the band structure in \Qref{sec:essloc}. These are the minimal assumptions one needs to impose on systems in the present setting. On the one hand, locality is crucial in order to speak of a physical system and on the other continuity is needed in order to formulate quantities like winding numbers of the bands. Therefore we consider it a remarkable fact, that these assumptions actually coincide.

In \Qref{sec:classification} we give the complete homotopy classification of translation invariant quantum walks for the symmetry types \symD, \symAIII, \symBDI, \symCII and \symDIII. The section is divided into three parts, where in the first part we address quantum walks with only particle hole symmetry (\symD), in the second part those with a chiral symmetry, which squares to $+\idty$ (\symAIII, \symBDI and \symCII) and finally we address walks of symmetry type \symDIII in the third part. For each of these symmetry types we derive an index formula in terms of winding numbers. For continuously differentiable band structures we derive Berry-type integrals for every symmetry type under consideration.

Each part in \Qref{sec:classification} is followed by a discussion about completeness of the respective invariants under consideration. Results on completeness always depend critically on the assumptions one demands to be fulfilled along the transformation. Of course the general theory also covers translation invariant walks, but it might be possible that one has to leave this set in order to construct homotopies. Hence, the question of whether two translation invariant walks with the same symmetry indices can be continuously connected with each other in the set of translation invariant walks is left open by \cite{LongVersion}.
Here we show that the completeness result in \cite{LongVersion} still holds for the symmetry types \symAIII, \symCII and \symDIII. For the types \symD and \symBDI additional invariants emerges, which strongly depend on a fixed cell structure. Indeed it turns out that these new invariants trivialize, if we allow for regrouping of neighbouring cells or the addition of trivial ancillary systems.

Finally we address the question how eigenfunction at the edge of translation invariant walks decay in the bulk. It is generally assumed, that such functions have to decay exponentially but we could not find a reference where this is actually shown. In \Qref{sec:decay} we prove, that this is indeed the case. 



